Near optimal sparsity-constrained group testing: improved bounds and algorithms

Recent advances in noiseless non-adaptive group testing have led to a precise asymptotic characterization of the number of tests required for high-probability recovery in the sublinear regime $k = n^{\theta}$ (with $\theta \in (0,1)$), with $n$ individuals among which $k$ are infected. However, the required number of tests may increase substantially under real-world practical constraints, notably including bounds on the maximum number $\Delta$ of tests an individual can be placed in, or the maximum number $\Gamma$ of individuals in a given test. While previous works have given recovery guarantees for these settings, significant gaps remain between the achievability and converse bounds. In this paper, we substantially or completely close several of the most prominent gaps. In the case of $\Delta$-divisible items, we show that the definite defectives (DD) algorithm coupled with a random regular design is asymptotically optimal in dense scaling regimes, and optimal to within a factor of $\eul$ more generally; we establish this by strengthening both the best known achievability and converse bounds. In the case of $\Gamma$-sized tests, we provide a comprehensive analysis of the regime $\Gamma = \Theta(1)$, and again establish a precise threshold proving the asymptotic optimality of SCOMP (a slight refinement of DD) equipped with a tailored pooling scheme. Finally, for each of these two settings, we provide near-optimal adaptive algorithms based on sequential splitting, and provably demonstrate gaps between the performance of optimal adaptive and non-adaptive algorithms.

==> b_SavedFigs.tex <==
\IEEEcompsocitemizethanks{\IEEEcompsocthanksitem Oliver Gebhard,  oliver.gebhard@tu-dortmund.de, Faculty of Computer Science, TU Dortmund University, Dortmund, Germany, 44227.\protect\\
\IEEEcompsocthanksitem  Max Hahn-Klimroth,  maximilian.hahnklimroth@tu-dortmund.de, Faculty of Computer Science, TU Dortmund University, Dortmund, Germany, 44227.\protect\\
\IEEEcompsocthanksitem Olaf Parczyk,  parczyk@mi.fu-berlin.de, Department of Mathematics and Computer Science, FU Berlin, Berlin, Germany, 14195. \protect\\
\IEEEcompsocthanksitem Manuel Penschuck,  manuel@ae.cs.uni-frankfurt.de, Institute of Computer Science, Goethe University Frankfurt, Frankfurt, Germany, 60325. \protect\\
\IEEEcompsocthanksitem Maurice Rolvien,  maurice.rolvien@tu-dortmund.de, Faculty of Computer Science, TU Dortmund University, Dortmund, Germany, 44227.\protect\\
\IEEEcompsocthanksitem Jonathan Scarlett, scarlett@comp.nus.edu.sg, Department of Computer Science, National University of Singapore, Singapore, 117418. \protect\\
\IEEEcompsocthanksitem Nelvin Tan,  tcnt2@cam.ac.uk, Department of Engineering, University of Cambridge, UK, CB2 1PZ.\protect\\
}

\begin{figure}
    \hspace{1.25cm}
    \begin{minipage}[t][][b]{0.7 \textwidth}
        \begin{tikzpicture}[scale=0.7]
            \begin{axis}[
                axis lines = left,
                xlabel = density parameter $\theta$,
                ylabel style={at={(0,0.3)}},
                xtick={0, 0.5 - 5/(2*11.513), 0.5, 1},
                xticklabels={$0$, $1/2 - \Delta/(2 \log n)$, $1/2$, $1$},
                ytick={1.2},
                yticklabels={$1+\frac{1}{\Delta}$},
                ymin = 0,
                ymax = 6.0,
                xmin = 0,
                xmax=1.05,
                height=7.1cm,
                width=13.5cm,
                legend style={at={(axis cs:0.3,5.99)},anchor=north west},
                x label style={at={(axis description cs:0.7,-0.2)},anchor=north},
                font = \small
                ]
                
                \addplot [
                name path=minf,
                domain=0:1, 
                samples=100, 
                style={ultra thick},
                solid,
                color=black,
                ]
                {1.0 + (1-x)/(5*x) - 1/(x * 11.513)};
                \addlegendentry{Universal Lower Bound}
                
                \addplot [
                name path=madaalg,
                domain=0:1, 
                samples=100, 
                style={ultra thick},
                dotted,
                color=orange,
                ]
                {1.0 + (1-x)/(5*x)};
                \addlegendentry{Adaptive Algorithm}
                
                
                
                \addplot [
                name path=mdd,
                domain=0:1, 
                samples=100, 
                color=blue,
                style={ultra thick},
                dashed
                ]
                {max(1.2, 1 + (1-x)/( 5*x )};
                \addlegendentry{DD Upper Bound}
                %\addlegendentry{$\tilde m_{\text{DD}}(\Delta)$}
                
                \addplot [
                name path=mnonada,
                domain=0:1, 
                samples=100, 
                color=red,
                style={ultra thick},
                dashed
                ]
                {max(1.2, 1 + (1-x)/( 5*x ) - 1/(x * 11.513)};
                \addlegendentry{Non-Adaptive Lower Bound}
                
                \addplot [
                name path=mcomp,
                domain=0:1, 
                samples=100, 
                color=green,
                style={ultra thick},
                dashed
                ]
                {1.0 + 1/(5*x) + 1/(x*11.513)};
                \addlegendentry{COMP Upper Bound}
                
                
                
                \addplot [
                name path=border_up,
                domain=0:1, 
                samples=10, 
                color=purple,
                style={thin},
                draw opacity=0.00,
                dashed
                ]
                {3.0+0.001};
                
                
                \addplot [
                name path=border_low,
                domain=0:1, 
                samples=10, 
                color=purple,
                style={thin},
                draw opacity=0.00,
                dashed
                ]
                {0.001};
                
                
                \addplot [
                thick,
                color=white,
                fill=white, 
                fill opacity=0.5
                ]
                fill between[
                of=minf and border_low,
                soft clip={domain=0:1},
                ];
                
                \addplot [
                thick,
                color=purple,
                fill=white, 
                fill opacity=0.5
                ]
                fill between[
                of=minf and madaalg,
                soft clip={domain=0:1},
                ];
                
                \addplot [
                thick,
                color=purple,
                fill=white, 
                fill opacity=0.5
                ]
                fill between[
                of=minf and mnonada,
                soft clip={domain=0.28285416:0.5},
                ];
                
                \addplot [
                thick,
                color=purple,
                fill=white, 
                fill opacity=0.5
                ]
                fill between[
                of=minf and madaalg,
                soft clip={domain=0.5:1},
                ];
                
                
                
                \addplot [
                thick,
                color=purple,
                fill=white, 
                fill opacity=0.3
                ]
                fill between[
                of=mnonada and mdd,
                soft clip={domain=0:0.5},
                ];
                
                \addplot [
                thick,
                color=green,
                fill=white, 
                fill opacity=0.2
                ]
                fill between[
                of=mdd and mcomp,
                soft clip={domain=0:1},
                ];
                
                
                
                \addplot [
                thick,
                color=green,
                fill=white, 
                fill opacity=0.5
                ]
                fill between[
                of=mcomp and border_up,
                soft clip={domain=0:1},
                ];
                
                \addplot [
                thick,
                color=purple,
                fill=white, 
                fill opacity=0.3
                ]
                fill between[
                of=madaalg and mdd,
                soft clip={domain=0.5:1},
                ];
                
                
                % \path[name path=axis] (axis cs:0,0) -- (axis cs:1,0);
                
                \addplot+[
                mark=none,
                color=purple,
                dotted,
                ]
                coordinates
                {(0,1.2) (0.5 - 5/(2*11.513), 1.2)};
                
                \addplot+[
                mark=none,
                color=purple,
                dotted,
                ]
                coordinates
                {(0.5 - 5/(2*11.513),0) (0.5 - 5/(2*11.513),1.2)};
                
                \addplot+[
                mark=none,
                color=purple,
                dotted,
                ]
                coordinates
                {(0.5, 0) (0.5,1.2)};
                
            \end{axis}
            
        \end{tikzpicture}
        
    \end{minipage}
    
    \caption{\geb{Illustration of values of $c$ such that $m = \Delta k^{c(1+o(1))}$} for the $\Delta-$divisible setting with $\Delta = 5$ and $n = 10^5$. }
    \label{fig_bounds_illustration_delta_divisible}
\end{figure}
%This figure was modified from \cite{phd_thesis_max}.
\begin{figure}
    % \hspace{-4.5cm}
    \begin{minipage}{0.55 \textwidth}
        
        \begin{tikzpicture}[scale=0.7]
            \begin{axis}[
                axis lines = left,
                xlabel = density parameter $\theta$,
                ylabel style={at={(0,0.3)}},
                xtick={0, 0.5, 1},
                xticklabels={$0$, $1/2$, $1$},
                ytick={1,2,3,4},
                yticklabels={$1$, $2$, $3$, $4$},
                ymin = 0,
                ymax = 4.5,
                xmin = 0,
                xmax=1.05,
                height=9.0cm,
                width=15.5cm,
                legend style={at={(axis cs:0.02,4.7)},anchor=north west},
                x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
                font = \small
                ]
                
                \addplot [
                name path=minf,
                domain=0:1, 
                samples=100, 
                style={ultra thick},
                solid,
                color=black,
                ]
                {1.0};
                \addlegendentry[scale=1.4]{Universal Lower Bound}
                
                \addplot [
                name path=mnonada,
                jump mark mid,
                domain=0:0.91, 
                samples=100, 
                color=red,
                clip = false,
                style={ultra thick},
                dashed
                ]
                {min(max( 1 + floor(x/(1-x)), 2*4/5), 4)};
                \addlegendentry[scale=1.4]{Non adaptive Lower Bound}
                
                \addplot [
                name path=mnonada,
                jump mark mid,
                domain=0:0.91, 
                samples=100, 
                color=blue,
                clip = false,
                style={ultra thick},
                dotted
                ]
                {min(max( 1 + floor(x/(1-x)), 2*4/5), 4)};
                \addlegendentry[scale=1.4]{DD Upper Bound}
                
                \addplot [
                name path=comp,
                jump mark mid,
                domain=0:0.91, 
                samples=100, 
                clip= false,
                color=green,
                style={ultra thick},
                dotted
                ]
                {min(ceil(1/(1-x)), 4)};
                \addlegendentry[scale=1.4]{COMP Upper Bound}
                
                
                
                
                \addplot [
                name path=border_up,
                domain=0:1, 
                samples=10, 
                color=purple,
                style={thin},
                draw opacity=0.00,
                solid
                ]
                {10.05};
                
                
                \addplot [
                name path=border_low,
                domain=0:1, 
                samples=10, 
                color=purple,
                style={thin},
                draw opacity=0.00,
                solid
                ]
                {0.001};
                
                
                
                
                \path[name path=axis] (axis cs:0,0) -- (axis cs:1.01,0);
                
                \addplot+[
                mark=none,
                color=purple,
                dotted,
                ]
                coordinates
                {(0.5,0) (0.5,2)};
                
            \end{axis}
            
        \end{tikzpicture}
        
    \end{minipage}
    
    \caption{\geb{Illustration of thresholds $c$ such that $m = (c+o(1)) \frac{n}{\Gamma}$} under $\Gamma-$sparse tests, with $\Gamma = 4$. \geb{The adaptive algorithmic bound (not shown) coincides with the universal lower bound, and {\tt DD} matches the non-adaptive lower bound except possibly at the discontinuities.}}
    %This figure was modified from \cite{phd_thesis_max}.
    \label{fig_bounds_illustration_gamma_sparse}
\end{figure}

==> tikz_graphics.tex <==
\newcommand\FigPhaseTransitionsGTDelta{
\begin{figure}[ht]
\begin{minipage}[t][][b]{0.95 \textwidth}
\adjustbox{center}{
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
axis lines = left,
 xlabel = density parameter $\theta$,
ylabel style={at={(0,0.3)}},
xtick={0, 0.5 - 5/(2*11.513), 0.5, 1},
xticklabels={$0$, $\frac{1}{2} - \frac{\Delta}{2 \log n}$, $\frac{1}{2}$, $1$},
ytick={1.2},
yticklabels={$1+\frac{1}{\Delta}$},
ymin = 0,
ymax = 3.0,
xmin = 0,
xmax=1.05,
height=7.1cm,
width=13.5cm,
legend style={at={(axis cs:1.01,2.99)},anchor=north west},
x label style={at={(axis description cs:0.9,-0.1)},anchor=north},
font = \small
]

\addplot [
name path=minf,
domain=0:1, 
samples=100, 
style={ultra thick},
solid,
color=purple,
]
{1.0 + (1-x)/(5*x) - 1/(x * 11.513)};
\addlegendentry{$\tilde m_{\text{inf}}(\Delta)$}

\addplot [
name path=madaalg,
domain=0:1, 
samples=100, 
style={ultra thick},
dotted,
color=orange!70,
]
{1.0 + (1-x)/(5*x)};
\addlegendentry{$\tilde m_{\text{ada-alg}}(\Delta)$}



\addplot [
name path=mdd,
domain=0:1, 
samples=100, 
color=green!50,
style={ultra thick},
dashed
]
{max(1.2, 1 + (1-x)/( 5*x )};
\addlegendentry{$\tilde m_{\text{DD}}(\Delta)$}


\addplot [
name path=mnonada,
domain=0:1, 
samples=100, 
color=red,
style={ultra thick},
dashed
]
{max(1.2, 1 + (1-x)/( 5*x ) - 1/(x * 11.513)};
\addlegendentry{$\tilde m_{\text{non-ada}}(\Delta)$}

\addplot [
name path=mcomp,
domain=0:1, 
samples=100, 
color=green,
style={ultra thick},
dashed
]
{1.0 + 1/(5*x) + 1/(x*11.513)};
\addlegendentry{$\tilde m_{\text{COMP, G}}(\Delta)$}



\addplot [
name path=border_up,
domain=0:1, 
samples=10, 
color=purple,
style={thin},
draw opacity=0.00,
dashed
]
{3.0+0.001};


\addplot [
name path=border_low,
domain=0:1, 
samples=10, 
color=purple,
style={thin},
draw opacity=0.00,
dashed
]
{0.001};


\addplot [
        thick,
        color=white,
        fill=red, 
        fill opacity=0.5
    ]
    fill between[
        of=minf and border_low,
        soft clip={domain=0:1},
    ];

\addplot [
        thick,
        color=purple,
        fill=yellow, 
        fill opacity=0.5
    ]
    fill between[
        of=minf and madaalg,
        soft clip={domain=0:1},
    ];

\addplot [
        thick,
        color=purple,
        fill=orange!70, 
        fill opacity=0.5
    ]
    fill between[
        of=minf and mnonada,
        soft clip={domain=0.28285416:0.5},
    ];
    
\addplot [
        thick,
        color=purple,
        fill=orange!70, 
        fill opacity=0.5
    ]
    fill between[
        of=minf and madaalg,
        soft clip={domain=0.5:1},
    ];
    


\addplot [
        thick,
        color=purple,
        fill=yellow, 
        fill opacity=0.3
    ]
    fill between[
        of=mnonada and mdd,
        soft clip={domain=0:0.5},
    ];

\addplot [
        thick,
        color=green,
        fill=green, 
        fill opacity=0.2
    ]
    fill between[
        of=mdd and mcomp,
        soft clip={domain=0:1},
    ];



\addplot [
        thick,
        color=green,
        fill=green, 
        fill opacity=0.5
    ]
    fill between[
        of=mcomp and border_up,
        soft clip={domain=0:1},
    ];
    
\addplot [
        thick,
        color=purple,
        fill=red, 
        fill opacity=0.3
    ]
    fill between[
        of=madaalg and mdd,
        soft clip={domain=0.5:1},
    ];


% \path[name path=axis] (axis cs:0,0) -- (axis cs:1,0);

\addplot+[
mark=none,
color=purple,
dotted,
]
coordinates
{(0,1.2) (0.5 - 5/(2*11.513), 1.2)};

\addplot+[
mark=none,
color=purple,
dotted,
]
coordinates
{(0.5 - 5/(2*11.513),0) (0.5 - 5/(2*11.513),1.2)};

\addplot+[
mark=none,
color=purple,
dotted,
]
coordinates
{(0.5, 0) (0.5,1.2)};

\end{axis}

\end{tikzpicture}
}
\end{minipage}

\caption{Phase diagram for the $\Delta-$divisible setting at the example  $\Delta = 5$, $n = 10^5$ such that $m = \Delta k^{\tilde m}$. Modified after \cite{phd_thesis_max}}
\label{fig_bounds_illustration_delta_divisible}
\end{figure}

}



\newcommand\FigPhaseTransitionsGTGammaSparse{

\begin{figure}[ht]
\begin{minipage}[t][][b]{0.95 \textwidth}
\adjustbox{center}{
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
axis lines = left,
 xlabel = density parameter $\theta$,
ylabel style={at={(0,0.3)}},
xtick={0, 0.5, 1},
xticklabels={$0$, $\frac{1}{2}$, $1$},
ytick={1,2,3,4},
yticklabels={$1$, $2$, $3$, $4$},
ymin = 0,
ymax = 4.5,
xmin = 0,
xmax=1.05,
height=9.0cm,
width=16.5cm,
legend style={at={(axis cs:1.01,4.49)},anchor=north west},
x label style={at={(axis description cs:0.9,-0.1)},anchor=north},
font = \small
]

\addplot [
name path=minf,
domain=0:1, 
samples=100, 
style={ultra thick},
solid,
color=purple,
]
{1.0};
\addlegendentry{$\tilde m_{\text{inf}}(\Gamma)$}

\addplot [
name path=mnonada,
jump mark mid,
domain=0:0.91, 
samples=100, 
color=red,
clip = false,
style={ultra thick},
solid
]
{min(max( 1 + floor(x/(1-x)), 2*4/5), 4)};
\addlegendentry{$\tilde m_{\text{non-ada}}(\Gamma)$}



\addplot [
name path=comp,
jump mark mid,
domain=0:0.91, 
samples=100, 
clip= false,
color=green,
style={ultra thick},
dotted
]
{min(ceil(1/(1-x)), 4)};
\addlegendentry{$\tilde m_{\text{COMP, G}}(\Gamma)$}




\addplot [
name path=border_up,
domain=0:1, 
samples=10, 
color=purple,
style={thin},
draw opacity=0.00,
solid
]
{10.05};


\addplot [
name path=border_low,
domain=0:1, 
samples=10, 
color=purple,
style={thin},
draw opacity=0.00,
solid
]
{0.001};




\path[name path=axis] (axis cs:0,0) -- (axis cs:1.01,0);

\addplot+[
mark=none,
color=purple,
dotted,
]
coordinates
{(0.5,0) (0.5,2)};

\end{axis}

\end{tikzpicture}
}
\end{minipage}

\caption{Phase-transitions under the $\Gamma-$sparse restriction for $\Gamma = \Theta(1)$ with $m = \tilde m \frac{n}{\Gamma}$. The plot is with respect to $\Gamma = 4$. Modified after \cite{phd_thesis_max}.
\label{fig_bounds_illustration_gamma_sparse}
\end{figure}

}
